Pelphix: Surgical Phase Recognition from X-ray Images in Percutaneous Pelvic Fixation

Surgical phase recognition (SPR) is a crucial element in the digital transformation of the modern operating theater. While SPR based on video sources is well-established, incorporation of interventional X-ray sequences has not yet been explored. This paper presents Pelphix, a first approach to SPR for X-ray-guided percutaneous pelvic fracture fixation, which models the procedure at four levels of granularity -- corridor, activity, view, and frame value -- simulating the pelvic fracture fixation workflow as a Markov process to provide fully annotated training data. Using added supervision from detection of bony corridors, tools, and anatomy, we learn image representations that are fed into a transformer model to regress surgical phases at the four granularity levels. Our approach demonstrates the feasibility of X-ray-based SPR, achieving an average accuracy of 93.8% on simulated sequences and 67.57% in cadaver across all granularity levels, with up to 88% accuracy for the target corridor in real data. This work constitutes the first step toward SPR for the X-ray domain, establishing an approach to categorizing phases in X-ray-guided surgery, simulating realistic image sequences to enable machine learning model development, and demonstrating that this approach is feasible for the analysis of real procedures. As X-ray-based SPR continues to mature, it will benefit procedures in orthopedic surgery, angiography, and interventional radiology by equipping intelligent surgical systems with situational awareness in the operating room.

==> citation_shorten.tex <==
\newcommand{\etal}{\textit{et al.}}

\newcommand{\authornames}[1]{%
    \ifthenelse{\value{listtotal} > 3}
    {\relax\expandafter\ifthenelse{\value{listcount}=1}{#1\etal}{\ifthenelse{\value{listcount}<\value{listtotal}}{, #1}{}.\etal}}%
    {\relax\expandafter\ifthenelse{\value{listcount}=1}{#1}{\ifthenelse{\value{listcount}<\value{listtotal}}{, #1}{}.\ }}
}

